Effects of magnetic perturbations and radiation on the runaway avalanche

The electron runaway phenomenon in plasmas depends sensitively on the momentum-space dynamics. However, efficient simulation of the global evolution of systems involving runaway electrons typically requires a reduced fluid description. This is needed for example in the design of essential runaway mitigation methods for tokamaks. In this paper, we present a method to include the effect of momentum-dependent spatial transport in the runaway avalanche growth rate. We quantify the reduction of the growth rate in the presence of electron diffusion in stochastic magnetic fields and show that the spatial transport can raise the effective critical electric field. Using a perturbative approach we derive a set of equations that allows treatment of the effect of spatial transport on runaway dynamics in the presence of radial variation in plasma parameters. This is then used to demonstrate the effect of spatial transport in current quench simulations for ITER-like plasmas with massive material injection. We find that in scenarios with sufficiently slow current quench, due to moderate impurity and deuterium injection, the presence of magnetic perturbations reduces the final runaway current considerably. Perturbations localized at the edge are not effective in suppressing the runaways, unless the runaway generation is off-axis, in which case they may lead to formation of strong current sheets at the interface of the confined and perturbed regions.

==> settings.tex <==
% CREATED BY DAVID FRISK, 2018

% BASIC SETTINGS
\usepackage[dvipsnames]{xcolor}
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage[T1]{fontenc}							% Output settings
\usepackage[english]{babel}							% Language settings
\usepackage[utf8]{inputenc}							% Input settings
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}								% Figures
\usepackage{subfig}									% Enables subfigures
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{listings}								% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage{chemformula}

\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage{pgfplots}
\pgfplotsset{compat=1.3}
\pgfplotsset{plot coordinates/math parser=false}
\newlength\figureheight
\newlength\figurewidth
\usepackage{nicefrac}

% Fixes footnotes
\interfootnotelinepenalty=10000

\usepackage[style=phys, biblabel=brackets]{biblatex}
%\usepackage[style=numeric]{biblatex}
\setlength\bibitemsep{0.2\baselineskip}
\addbibresource{include/backmatter/ref.bib}

\usepackage{letltxmacro}
\LetLtxMacro{\oldcite}{\cite}
\renewcommand{\cite}[1]{\mbox{\oldcite{#1}}}

% My own defined commands.
\newcommand{\deri}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dt}[1]{\deri{#1}{t}}
\newcommand{\derip}[1]{\deri{#1}{p}}
\newcommand{\dlambda}[1]{\deri{#1}{\lambda}}
\newcommand{\diff}[2]{\frac{1}{r}\frac{\partial}{\partial r}r#1 \frac{\partial #2}{\partial r}}
\newcommand{\diffx}[2]{\frac{1}{x}\frac{\partial}{\partial x}x#1 \frac{\partial #2}{\partial x}}
\newcommand{\loglambda}{\ln \Lambda}
\newcommand{\pperp}{p_{\perp}}
\newcommand{\ppar}{p_{||}}
\newcommand{\F}[3]{F_{#1, #2}^{#3}}
\newcommand{\dd}[3]{\left(\nu_d\right)_{#1, #2}^{#3}}
\newcommand{\E}[2]{E_{#1}^{#2}}
\newcommand{\pmax}{p_{\text{max}}}
\newcommand{\pref}{p_{\text{ref}}}
\newcommand{\hf}{\mathcal{H}}
\newcommand{\Gf}{\mathcal{G}}
\newcommand{\Eceff}{E_c^{\text{eff}}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\mathbb{#1}}
\DeclareMathOperator\erf{erf}

% Ola :-)
\newcommand{\idea}{\color{OliveGreen}}
%\newcommand{\idea}{\color{black}}
%\newcommand{\partway}{\color{blue}}
\newcommand{\partway}{\color{black}}
\newcommand{\redy}{\color{black}}
\newcommand{\note}[1]{\textcolor{red}{#1}}

% Show label in the pdf
%\usepackage[inline]{showlabels}
\usepackage[final]{showlabels}



% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)

% Disable automatic indentation (equal to using \noindent)
\setlength{\parindent}{0cm}                         


% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption} 		

		  	
% Activate clickable links in table of contents  	
\usepackage{hyperref}								
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}


% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{5}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]


% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{2}	% Choose 1 for one-sided or 2 for two-sided layout
% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi


% Enable To-do notes
\usepackage[textsize=tiny]{todonotes}   % Include the option "disable" to hide all notes
\setlength{\marginparwidth}{2.5cm} 


% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		


% Tag command (invisible)
\newcommand{\tagtemp}{\textcolor{white}{, template by David Frisk}}




